Building A Coding Assistant via the Retrieval-Augmented Language Model

Pretrained language models have shown strong effectiveness in code-related tasks, such as code retrieval, code generation, code summarization, and code completion tasks. In this paper, we propose COde assistaNt viA retrieval-augmeNted language model (CONAN), which aims to build a code assistant by mimicking the knowledge-seeking behaviors of humans during coding. Specifically, it consists of a code structure aware retriever (CONAN-R) and a dual-view code representation-based retrieval-augmented generation model (CONAN-G). CONAN-R pretrains CodeT5 using Code-Documentation Alignment and Masked Entity Prediction tasks to make language models code structure-aware and learn effective representations for code snippets and documentation. Then CONAN-G designs a dual-view code representation mechanism for implementing a retrieval-augmented code generation model. CONAN-G regards the code documentation descriptions as prompts, which help language models better understand the code semantics. Our experiments show that CONAN achieves convincing performance on different code generation tasks and significantly outperforms previous retrieval augmented code generation models. Our further analyses show that CONAN learns tailored representations for both code snippets and documentation by aligning code-documentation data pairs and capturing structural semantics by masking and predicting entities in the code data. Additionally, the retrieved code snippets and documentation provide necessary information from both program language and natural language to assist the code generation process. CONAN can also be used as an assistant for Large Language Models (LLMs), providing LLMs with external knowledge in shorter code document lengths to improve their effectiveness on various code tasks. It shows the ability of CONAN to extract necessary information and help filter out the noise from retrieved code documents.

==> tables/analysis_com.tex <==
\begin{table*}[t]
\centering
\small
\caption{}
\label{tab:analysis_com}
\begin{tabular}{c|cc|cc}
\hline
\textbf{Methods} & \multicolumn{2}{c|}{\textbf{PY150}}                & \multicolumn{2}{c}{\textbf{JavaCorpus}}            \\ \hline
Name             & \multicolumn{1}{c|}{Exact Match}   & Edit Sim      & \multicolumn{1}{c|}{Exact Match}   & Edit Sim      \\ \hline
CONAN      & \multicolumn{1}{c|}{\textbf{40.1}} & \textbf{69.4} & \multicolumn{1}{c|}{26.0}          & \textbf{62.7} \\
CodeT5(concat)   & \multicolumn{1}{c|}{39.9}          & 67.4          & \multicolumn{1}{c|}{25.4}          & 60.2          \\
CodeT5(single)   & \multicolumn{1}{c|}{38.7}          & 68.4          & \multicolumn{1}{c|}{\textbf{26.5}} & 60.9          \\ \hline
\end{tabular}
\end{table*}

==> tables/analysis_gen.tex <==
\begin{table*}[t]
\centering
\small
\caption{}
\label{tab:analysis_gen}
\begin{tabular}{c|ccc|ccc|ccc}
\hline
\textbf{Methods} & \multicolumn{3}{c|}{\textbf{CSN-Python}}      & \multicolumn{3}{c|}{\textbf{CSN-Java}}        & \multicolumn{3}{c}{\textbf{Concode}}          \\ \hline
Name             & EM            & BLEU          & CodeBLEU      & EM            & BLEU          & CodeBLEU      & EM            & BLEU          & CodeBLEU      \\ \hline
CONAN            & \textbf{14.6} & \textbf{32.9} & \textbf{37.3} & \textbf{17.2} & \textbf{37.7} & \textbf{45.4} & \textbf{23.1} & 42.8          & \textbf{45.1} \\
CodeT5(Concat)   & 12.3          & 27.5          & 31.7          & 13.0          & 32.0          & 36.5          & 23.1          & 41.9          & 44.7          \\
CodeT5(Single)   & 13.1          & 30.3          & 35.0          & 15.4          & 35.0          & 41.8          & 23.1          & \textbf{42.9} & 44.9          \\ \hline
\end{tabular}
\end{table*}

==> tables/analysis_sum.tex <==
\begin{table}[t]
\centering
\small
\caption{}
\label{tab:analysis_sum}
\begin{tabular}{c|c|c}
\hline
\textbf{Methods} & \textbf{Python} & \textbf{Java} \\ \hline
CONAN            & \textbf{23.5}   & \textbf{26.5} \\ \hline
CodeT5(Concat)   & 22.1            & 23.8          \\ \hline
CodeT5(Single)   & 23.4            & 25.9          \\ \hline
\end{tabular}
\end{table}

==> tables/case_new.tex <==
% \begin{table}[t]
%     \centering
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{lp{15cm}}
%         \toprule
%         \textbf{Code Generation \hspace{0.3cm}} &  \\
%         \midrule
%         \texttt{Input} & Fetches a field from extras and returns it. This is some Airflow magic. The grpc hook type adds custom UI elements to the hook page which allow admins to specify scopes credential pem files etc. They get formatted as shown below. \\
        
%         \midrule
%         \texttt{REDCODER} & Top-1:\hfill \break\ 
%         \includegraphics[width=0.9\textwidth]{figures/image/connan_top1.png}
     
%                         \hfill \break
% Prediction:\hfill \break
% \includegraphics[width=0.9\textwidth]{figures/image/connan_top1.png} \\

%         \midrule
%         \texttt{\textbf{CONAN}} & Top-1:\hfill \break\ \includegraphics[width=0.9\textwidth]{figures/image/connan_top1.png}
%                         \hfill \break
% Prediction:\hfill \break
% \includegraphics[width=0.9\textwidth]{figures/image/connan_top1.png}\\

%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Case studies on code generation task.}
% \end{table}


% \begin{table}[h!]
%     \centering
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{lp{15cm}}
%         \toprule
%         \textbf{Code Summarization} &  \\
%         \midrule
%         \texttt{Input} & \hfill \break \includegraphics[width=0.9\textwidth]{figures/image/connan_top1.png} \\
%         \texttt{REDCODER} & Top-1: xxx
%                         \hfill \break\hfill \break
% Prediction:xxx \\

%         \midrule
%         \texttt{\textbf{CONAN}} & Top-1: xxx
%                         \hfill \break\hfill \break
% Prediction:xxx \\

%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Case studies on code summarization task.}
% \end{table}


% \begin{table}[h!]
%     \centering
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{lp{15cm}}
%         \toprule
%         \textbf{Code Completion\hspace{0.5cm}} &  \\
%         \midrule
%         \texttt{Input} & Retrieves connection to Cloud Translate. \\
%         \midrule
%         \texttt{CodeGPT} & xxx \\
%         \midrule
%         \texttt{CodeT5} & xxx \\
%         \midrule
%         \texttt{ReACC} & Top-1: xxx
%                         \hfill \break\hfill \break
% Prediction:xxx \\

%         \midrule
%         \texttt{\textbf{CONAN}} & Top-1: xxx
%                         \hfill \break\hfill \break
% Prediction:xxx \\

%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Case studies on code completion task.}
% \end{table}

==> tables/generation_concode.tex <==
\begin{table}[]
\centering
\small
\caption{Code Generation Results on Concode Dataset.}
\label{tab:gen_concode}
\scalebox{1}{
\begin{tabular}{lccc}
\hline
\multicolumn{1}{l|}{Methods}            & EM   & BLEU          & CodeBLEU \\ \hline
\multicolumn{4}{l}{Retrieval based}                               \\ \hline
\multicolumn{1}{l|}{BM25}               & 0    & 20.3          & 23.7     \\
\multicolumn{1}{l|}{SCODE-R}            & 0    & 32.6          & 36.5     \\
% \multicolumn{1}{l|}{CONAN-R(zero-shot)}      & 0    & 19.78         & 30.8     \\ 
\multicolumn{1}{l|}{CONAN-R}      & 0    & \textbf{33.5}         & \textbf{37.5}     \\ \hline
\multicolumn{4}{l}{Generative}                                    \\ \hline
\multicolumn{1}{l|}{Seq2Seq}            & 3.1  & 21.3          & 26.4     \\
\multicolumn{1}{l|}{Guo et al. (2019)}  & 10.1 & 24.4          & 29.5     \\
\multicolumn{1}{l|}{Iyer et al. (2019)} & 12.2 & 26.6          & -        \\
\multicolumn{1}{l|}{GPT-2}              & 17.4 & 25.4          & 29.7     \\
\multicolumn{1}{l|}{CodeGPT-2}          & 18.3 & 28.7          & 32.7     \\
\multicolumn{1}{l|}{CodeGPT-adapted}    & 20.1 & 32.8          & 36.0       \\
\multicolumn{1}{l|}{CodeBERT}           & 18.0   & 28.7          & 31.4     \\
\multicolumn{1}{l|}{GraphCodeBERT}      & 18.7 & 33.4          & 35.9     \\
\multicolumn{1}{l|}{PLBART}             & 18.6 & 36.7          & 38.5     \\
\multicolumn{1}{l|}{UniXcoder}          & 22.6 & 38.2         & -        \\
\multicolumn{1}{l|}{CodeT5(Paper)}      & 22.7 & 41.5         & 44.1     \\ 
\multicolumn{1}{l|}{CodeT5(Ours)}        & 22.2 & 39.6         & 43.8    \\ \hline
\multicolumn{4}{l}{Retrieval augmented generative}                \\ \hline
\multicolumn{1}{l|}{BM25+PLBART}        & 21.4 & 40.2          & 41.8     \\
\multicolumn{1}{l|}{REDCODER}           & \textbf{23.4} & 41.6          & 43.4     \\
\multicolumn{1}{l|}{REDCODER-EXT}       & 23.3 & 42.5 & 43.4     \\
\multicolumn{1}{l|}{CONAN}        & 23.1 & \textbf{42.8 }       &   \textbf{45.1}   \\ \hline
\end{tabular}
}
\end{table}


==> tables/retriever_ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\small
\caption{Ablation Study about Code Retriever}
\label{tab:retriever_ablation}
\scalebox{1}{
\begin{tabular}{lcccc}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{}}} & \multicolumn{2}{c}{\textbf{CodeSearch}} & \multicolumn{2}{c}{\textbf{Adv}} \\ \cline{2-5} 
\multicolumn{1}{c}{}                           & NL2Code            & Code2NL            & NL2Code         & Code2NL        \\ \hline
Our Retriever                                  & 73.7               & 75.4               & \textbf{47.68}  & \textbf{36.89} \\ \hline
w/o Code2NL                                    & \textbf{73.9}      & 74.4               & 47.27           & 36.35          \\
w/o NL2Code                                    & 71.5               & \textbf{77.7}      & 46.62           & 34.64          \\ \hline
\end{tabular}
}
\end{table*}

==> tables/summarization_csn.tex <==
\begin{table}[t]
\centering
\small
\caption{Evaluation BLEU-4 Score for Code Summarization on CsCSN.}
\label{tab:sum_csn}
\scalebox{1}{
\begin{tabular}{lcc}
\hline
Methods       & Pyhton                    & Java                      \\ \hline
\multicolumn{3}{l}{Retrieval based}                           \\ \hline
BM25          & 1.92                      & 1.82                      \\
SCODE-R       & 14.98                     & 15.87                     \\
% CONAN-R(zero-shot) & 12.34                     & 14.04                       \\
CONAN-R & \textbf{15.56}                    & \textbf{16.19}                      \\ \hline
\multicolumn{3}{l}{Generative}                                \\ \hline
Seq2Seq       & 15.93                     & 15.09                     \\
Transformer   & 15.81                     & 16.26                     \\
RoBERTa       & 18.14                     & 16.47                     \\
CodeBERT      & 19.06                     & 17.65                     \\
GraphCodeBERT & 17.98                     & 17.85                     \\
PLBART        & 19.30                      & 18.45                     \\
UniXcoder     & 19.30                      &  -                      \\
CodeT5        & 20.36                     & 20.46 \\ \hline
\multicolumn{3}{l}{Retrieval augmented generative}            \\ \hline
BM25+PLBART   & 19.57                     & 19.71                     \\
REDCODER      & 21.01                     & 22.94                     \\
REDCODER-EXT  & 20.91                     & 22.95                     \\
CONAN   & \textbf{23.50}                     & \textbf{26.46}                        \\ \hline
\end{tabular}
}
\end{table}
